Characterizing Fake News Targeting Corporations

Misinformation proliferates in the online sphere, with evident impacts on the political and social realms, influencing democratic discourse and posing risks to public health and safety. The corporate world is also a prime target for fake news dissemination. While recent studies have attempted to characterize corporate misinformation and its effects on companies, their findings often suffer from limitations due to qualitative or narrative approaches and a narrow focus on specific industries. To address this gap, we conducted an analysis utilizing social media quantitative methods and crowd-sourcing studies to investigate corporate misinformation across a diverse array of industries within the S\&P 500 companies. Our study reveals that corporate misinformation encompasses topics such as products, politics, and societal issues. We discovered companies affected by fake news also get reputable news coverage but less social media attention, leading to heightened negativity in social media comments, diminished stock growth, and increased stress mentions among employee reviews. Additionally, we observe that a company is not targeted by fake news all the time, but there are particular times when a critical mass of fake news emerges. These findings hold significant implications for regulators, business leaders, and investors, emphasizing the necessity to vigilantly monitor the escalating phenomenon of corporate misinformation.

==> 3data_saved.tex <==
% \begin{figure}[t]
% \centering
% \includegraphics[width=0.4\textwidth]{figs/Reddit_authors_vs_pop.png}
% \caption{\newtext{Reddit users versus state population.} }\label{fig:users_vs_pop}
% \end{figure}

% \section{Data and Methods}
% % pre ai
% % To understand and compare to what extent S\&P 500 companies are targeted by misinformation, we focused on the \emph{Reddit company comments with news articles} (\S\ref{sec:reddit}) and assessed the credibility of the articles using established \emph{fact-checking sources} (\S\ref{sec:newsarticles}). Whether a company is targeted by fake news might simply depend on whether the company is newsworthy. News might be driven by an external interest in the company, or by the internal affairs of its employees. External interest is often financially quantified as
% % \emph{stock growth} (\S\ref{sec:stocks}), while internal affairs  have so far been harder to characterize: to do so, we turned to a popular \emph{company review website, Glassdoor} (\S\ref{sec:glassdoor}).

% % ai
% \newtext{
% To examine and compare the susceptibility of S\&P 500 companies to misinformation, we collated four types of data. We collected Reddit company comments mentioning news articles (\S\ref{sec:reddit}). The credibility of these articles was evaluated utilizing established fact-checking sources (\S\ref{sec:newsarticles}). It is possible that a company's likelihood of being targeted by fake news may simply be related to its level of newsworthiness. This news coverage may stem from an external interest in the company, such as financial performance as measured by stock growth (\S\ref{sec:stocks}), or internal factors within the company. Internal company affairs  have so far been harder to characterize. To do so, we analyzed data from a reputable company review website, Glassdoor (\S\ref{sec:glassdoor}).}




% \subsection{Reddit Company Comments with News}\label{sec:reddit}
% We used publicly available Pushshift API \cite{baumgartner2020pushshift} to download the  Reddit comments from January 2016 to December 2019. We included all comments from all public and quarantined subreddits (e.g., r/the\_Donald). 
% Since we studied S\&P 500, we chose to focus only on the users who are from the U.S. 



% %for elimination of geographical or cultural bias. Hence, we needed to link users to the locations where they live in. 
% Reddit does not explicitly provide user location. However, it is possible to obtain reliable estimates \cite{balsamo2019firsthand}. Starting from a list of 2,844 location-based subreddits that map to one of the U.S. cities or states (e.g., r/newyork, r/california), we listed the users with at least 5 comments in those subreddits. If they had posted in multiple states, we assigned the user to the state with the majority of comments. In this way, we placed $\sim$3M users in one of the U.S. states. The number of Reddit users per state scaled linearly with the state’s population ($\beta$ = 1.01, $R^2$=0.84) showing a good geographic representativeness (Figure \ref{fig:users_vs_pop}). 

% During the four years 2016-2019, these users authored 1.4 billion comments. Of these comments, 8.23M (0.6\%) contained news links, of which 1.35M (16\%) mentioned also an S\&P 500 company (Table \ref{tab:reddit_stats}). Those comments contained 11.3M/1.3M total/unique links and had 262 (52.4\%) of the S\&P 500 companies mentioned \cite{wikisp}. Finally, we classified a Reddit comment as a fake news comment if it contained a URL to a domain that appeared in the list of fake news domains, which was defined using the credibility sources described next (\S\ref{sec:newsarticles}). In total, there were 12.8K fake Reddit comments mentioning S\&P 500 companies.
% %and their monthly numbers are shown in Figure \ref{fig:data_timeline}. 
% We can observe over the years, the median number of Reddit comments per month discussing corporate fake news is $408$ (Figure \ref{fig:data_timeline}).
% % 10.2M/1.4M total/unique links mentioned,
% % There were 10228367/1448350 unique links mentioned, and 256 (51.2\%) of the S\&P 500 companies.

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.5\textwidth]{figs/timeline_fake.png}
% \caption{\newtext{Monthly \# Reddit comments containing both a fake link and a company name} (median: 408, standard deviation: 136). The peaks observed in early 2017 and late 2018 were mainly caused by news about Google and  Facebook. They were accused to: not comply with the law requesting the removal of harmful content (Facebook), and use politically biased algorithms (Google). } % \todo{bold the x-axis and y-axis}
% %\refine{There is a ` steady state' of fake news discussions on Reddit: the mean and median number of comments mentioning fake news article are respectively 436 and 408 per month on Reddit, with the standard deviation of 136.}}
% \label{fig:data_timeline}
% \end{figure}


% \begin{table*}
% \begin{center}
% \caption{Statistics about Reddit comments mentioning companies and  news links present in the comments. \label{tab:reddit_stats}}
% \begin{tabular}{ l|rrrrrr } 
%  \hline
% \textbf{Type of comments} & \textbf{\# comments} & \textbf{\# users}  & \textbf{\# total links} & \textbf{\# unique links} & \textbf{\# domains} & \textbf{\# companies} \\  \midrule
%  comments by geolocated users in the U.S.	& 1.4B &  3M &   & &  & \\
% company comments  & 11.1M	& { {795K} }& & & & 262 \\
% %news comments & 8.2M	& 875K & 3.6M &  7.9K &  \\
% %fake news comments & 116K	& 45K & 60.8K &  933 &  \\
% company comments with news & 1.4M	& 322K & 11.3M & {1.3M} & 5.1K & 208 \\ % \texttt{\symbol{92}w} company name 
% company comments with fake news & 12.8K	& 6.3K & 145.5K & {{39.7K} }  & 316 & 114 \\\hline
% \end{tabular}
% \vspace{2em}
% %%%%%%%%%%%%%%%%%%%%
% \caption{\newtext{Statistics about Glassdoor reviews of S\&P 500 companies.} \label{tab:glassdoor_stats} }
% \begin{tabular}{ llllll } 
%  \hline
% \textbf{\# total reviews} & \textbf{\# US-based reviews} & \textbf{\# companies}  & \textbf{avg (min-max) rating} & \textbf{avg (min-max) stess score} &  \textbf{time period} \\  \midrule
%  713K & 440K &  399 &  3.37 (1.62-5) & 1.11\% (0-9.52\%) & 2008-2020 \\
% % company comments  & 11.1M	& { {795K} }& & & & 2008-2020 \\
% % %news comments & 8.2M	& 875K & 3.6M &  7.9K &  \\
% % %fake news comments & 116K	& 45K & 60.8K &  933 &  \\
% % company comments with news & 1.4M	& 322K & 11.3M & {1.3M} & 5.1K & 208 \\ % \texttt{\symbol{92}w} company name 
% % company comments with fake news & 12.8K	& 6.3K & 145.5K & {{39.7K} }  & 316 & 114 \\
% \hline
% \end{tabular}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \end{center}
% \end{table*}


% \subsection{News Credibility Sources}\label{sec:newsarticles}

% %\todo{news}

% % \begin{table}
% % \begin{center}
% % \begin{tabular}{ l|ll } 
% %  \hline
% % \textbf{Reddit Comments} & \textbf{\# comments} & \textbf{\# users} \\ \hline
% % geolocated in the U.S.	& 1.4B &  3M \\
% % \texttt{\symbol{92}w} any/fake link & 8.23M/116K	& 875K/45K \\
% % \texttt{\symbol{92}w} any/fake link \& company name & 1.35M/12.8K	& 322K/6.3K \\ \hline
% % \end{tabular}
% % \vspace{2em}\\
% % \begin{tabular}{ l|ll } 
% %  \hline
% % \textbf{\specialcell{News Articles in}} & \textbf{\# links} & \textbf{\# domains} \\ \midrule
% % \emph{{all comments}} &  & \\
% % any/fake	&  3.6M/60.8K &  7.9K/933 \\
% % \midrule
% % \emph{{comments \texttt{\symbol{92}w} company name}} &  & \\ 
% % \specialcell{any/fake} & 1.4M/39.9K & 5050/316 \\ \hline
% % %\texttt{\symbol{92}w} any/fake link \& company mention & 1.35M/12.8K	& 322K/6.3K \\ \hline
% % \end{tabular}
% % \caption{Statistics about: Reddit comments mentioning companies\emph{(top)}; and  news links present in the comments \emph{(bottom)}. \todo{these tables are hard. maybe one table reporting add FAKE REDDIT COMMENTS like in figure 1. ALSO COMPANIES TARGETED AND COMPANIES NOT TARGETED}}
% % \label{tab:reddit_stats}
% % \end{center}
% % \end{table}

% %\paragraph{Domain Credibility Labels}

% % pre-ai
% % We defined news credibility at the level of a publisher (domain). That is to say, all the news articles published on a fake/low credibility domain were considered as fake/low credibility. To obtain domain credibility labels, we took a list of news domains (i.e., publishers) commonly used in misinformation research \cite{bozarth2020higher}. Specifically, we labeled domains as reputable using the compiled lists from Alexa \cite{alexa}, Media Bias/Fact Check \cite{mediabias}, and Vargo et al.~\cite{vargo2018agenda}.  This resulted in 8.9K total reputable news sites. We labelled non-reputable domains using 5 lists: Media Bias/Fact Check, Zimdars list \cite{zimdars2016my}, PolitiFact \cite{gillin2018politifact}, the Daily Dot \cite{dailydot}, and Allcott, et al.~\cite{allcott2019trends}. By combining the labels coming from each of the five sources, we categorized a domain as fake if it had regularly published fabricated news articles. This resulted in a total of 933 fake news domains.
% % Upon this classification, we found that there were 1.35M Reddit comments that included 131.5K/39.9K total/unique fake news articles along with mentions of 114 (22.8\%) of the S\&P 500 companies (Table \ref{tab:reddit_stats}). 

% % ai
% We established the credibility of news at the level of the publisher (or domain). Specifically, all articles published on a domain deemed as fake or of low credibility were also considered fake or low credibility. To determine domain credibility, we utilized a commonly utilized list of news domains in misinformation research \cite{bozarth2020higher}. Specifically, we labeled domains as reputable using lists compiled by Alexa \cite{alexa}, Media Bias/Fact Check \cite{mediabias}, and Vargo et al.\cite{vargo2018agenda}. This resulted in a total of $8,900$ reputable news sites. Non-reputable domains were labeled using Media Bias/Fact Check and four additional sources: Zimdars list \cite{zimdars2016my}, PolitiFact \cite{gillin2018politifact}, the Daily Dot \cite{dailydot}, and Allcott, et al~\cite{allcott2019trends}. By merging the labels from each of these five sources, we classified a domain as fake if it had a history of publishing fabricated news articles. This resulted in a total of 933 fake news domains. Upon this classification, we found that 1.35 million Reddit comments included mentions of $131,500/39,900$ total/unique fake news articles, as well as mentions of $114 (22.8\%)$ of the S\&P 500 companies (as outlined in Table \ref{tab:reddit_stats}).



% \subsection{Company Stock Market Data}\label{sec:stocks}
% We collated the S\&P 500 stock market data, including the monthly adjusted closing prices from 2016 until 2019 for each company, from the Yahoo Finance portal~\cite{yahoo}.

% \subsection{Glassdoor Company Reviews}\label{sec:glassdoor}
% We acquired data regarding internal corporate affairs from 440K reviews of the S\&P 500 companies posted during the twelve years 2008-2020 on {Glassdoor\footnote{\url{https://www.glassdoor.com}}}, a popular company reviewing site. In 2021, there were $50M$ monthly visitors on the platform, and $70M$ reviews about $1.3M$ companies. Current and former employees of companies describe their job experience, ranging from interviews to salaries to workplace culture. All the reviews we collected were from U.S.-based employees. We also obtained the employee ratings of each company. 


% %We finally collected S\&P 500 stock market data  from the Yahoo Finance portal.\footnote{\url{https://finance.yahoo.com}} 


% %\subsection{Ratings and Stress Mentions in Glassdoor Reviews}
% \subsection{Computing Company Metrics} %\cliniccomm{[Matteo] connect a bit better to previous. this could be originallity: Glassdoor data use. }
% % Whether a company is targeted by fake news might simply depend on whether the company is newsworthy. News might be driven by external interest in the company, or by internal affairs of its employees. 
% % External interest is often financially quantified as
% % %Market perceptions are generally quantified by 
% % stock growth, while internal affairs 
% % %employee perceptions 
% % have so far been harder to characterize.
% %Only recently, such a perceptions have been captured by mining company reviews


% %\todo{motivate the use of stress. }
% %Company reviews, capturing the overall perception of employees of the company and their stress level, reflect a company's inside view. It has been found that employee perception and stress level can impact the employee's and ultimately company's performance \cite{motowidlo1986occupational}. 

% %Therefore, it would be interesting to explore whether the internal condition of a company is associated with that company being targeted by fake news.


% %\rev{To ensure quality reviews, the site employs the following three mechanisms. First, an automatic (proprietary) and manual content moderation system is paired with the possibility for users to flag content. Such a combined system partly prevents fake reviews (e.g., a company unfairly forcing employees to leave positive reviews). Second, every user wanting to browse others' content has to take the time to write one review. Since otherwise people tend to leave mostly polarizing (positive or negative) reviews on rating websites, this requirement encourages neutral reviews. This  partly prevents the so-called \emph{non-response bias} (a situation in which the opinions of respondents are very different from those of non-respondents). Third, the site allows for a maximum of one review per employee per company per year, preventing any employee from contributing a disproportionate number of reviews, discouraging \emph{sampling bias} (a situation in which the opinions of some members are more represented in the data than those of others).} These reviews have been recently used in studies exploring corporate culture at scale~\cite{das2020modeling,dekay2013peering,luo2016employee,ji2017corporate}. Table \ref{tab:example_reviews} shows example reviews of companies of each stress type.

% %\todo{}
% %\subsubsection{
% %\paragraph{Stress Mentions in Glassdoor Reviews}

% %
% %
% %MedDL was compared against two well-known entity extraction tools: MetaMap (a well-established tool \cite{aronson2010overview} and a de-facto baseline method for NLP studies related to health \cite{tutubalina2018medical}) and TaggerOne (a machine learning tool using semi-Markov models and a medical lexicon \cite{leaman2016taggerone}). The MedDL method achieved a strict/relaxed $F1$-score of $.71$/$.85$ when extracting symptoms (Figure S4), outperforming both MetaMap and TaggerOne by a large margin (the two have $F1$-scores of $.17/.48$ and $.31/.58$, respectively). Furthermore, MedDL has shown generalizability when applied on data from platforms different than those it was trained on  \marios{(e.g., on dream reports \cite{vscepanovic2022epidemic})}.
% %
% %
% %Our evaluation metric is $F1$ score, which is the harmonic mean of precision $P$ and recall $R$:  
% %\begin{equation}
% %F1 = 2 \frac{P \cdot R} { P + R }
% %\end{equation}
% %\begin{equation*}
% %P=\frac{\# \textrm{correctly classified medical entities}}{\# \textrm{total  entities classified as being medical}}
% %\end{equation*}
% %and
% %\begin{equation*}
% %R=\frac{\# \textrm{correctly classified medical entities}}{\# \textrm{total medical entities}},
% %\end{equation*}
% %where for strict $F1$ score, only the exact matches are counted as correct, and for relaxed $F1$ score, also partial matches are counted as correct.



% \begin{table*}[]
%     \centering
%     \scriptsize
%         \begin{tabular}{lSlll}
%         \toprule
%         {Metric} &  Formula &  Description & Distribution \\
%         \midrule
%         \texttt{\# Reddit comments (C, T)}  & ${\# \textrm{Reddit comments mentioning C during time period T}}$  &   public popularity & \includegraphics[height=0.5cm]{figs\#_Reddit_comments.png} \\
%         \texttt{\# Reddit comments per capita (C, T)}      &  $\frac{\# \textrm{Reddit comments mentioning C during time period T}}{\# \textrm{Glassdoor reviews of C during time period T}} $ &       corrected public popularity & \includegraphics[height=0.5cm]{figs/#_Reddit_comments_per_capita.png} \\
%         \texttt{external reputation score (C, T)}  & \newtext{1 - $\frac{\# \texttt{negative Reddit comments mentioning C in time period T}}{\# \texttt{total Reddit comments mentioning C in time period T} }$} &  \newtext{ positive/neutral mentions on social media} &  \includegraphics[height=0.5cm]{figs/Q-score.png}\\
%         \texttt{stock valuation (C, T)} & \textrm{adjusted closing prices at end of time period $T$ for company C} &   external investor perception &  \\
%         \texttt{stock growth (C)} & $ \frac{\texttt{stock valuation (C, 2019)}}{\texttt{stock valuation (C, 2014)}} $ &   external investor perception & \includegraphics[height=0.5cm]{figs/stock_growth.png} \\
%         \texttt{Glassdoor rating (C, T)}        &  $\textrm{Glassdoor overall rating of company C within time period T}$  &  internal perception & \includegraphics[height=0.5cm]{figs/Glassdoor_rating.png} \\
%         \texttt{internal employee stress score (C, T)}   &  $\frac{\# \textrm{Glassdoor reviews mentioning stress for company C within time period T}}{\# \textrm{total Glassdoor reviews for company C within time period T}}$  &  stress mentions by employees  & \includegraphics[height=0.5cm]{figs/stress_score.png} \\
%         \texttt{pFake (C, T)}  & $ \frac{\# \textrm{fake Reddit comments mentioning C during time period T}}{\# \textrm{Reddit comments mentioning C during time period T}} $ & \specialcell{probability of \texttt{C} being\\targeted by fake news} & \includegraphics[height=0.5cm]{figs/pFake.png} \\
%         %\texttt{misinformation shock}  & $ \frac{\textrm{\# of months with its $pFake$>$(mean(pFake)+2*std(pFake))$}}{\textrm{\# of months of the entire periods}} $ & \specialcell{number of collusive and \\concentrated misinformation attacks \todo{double check the distribution}} & \includegraphics[height=0.5cm]{figs/pFake.png} \\
%         \texttt{misinformation shock (C, T)}  & $\textrm{\# months with $pFake(C, T_{month})$>$(pFake(C, T)+2*std(pFake(C, T)))$}$ & \specialcell{number of concentrated \\ misinformation attacks} & \includegraphics[height=0.5cm]{figs/misinformation_shock.png} \\
%         \bottomrule
%         \end{tabular}
%     \caption{List of company metrics.}
%     %\todo{change color scheme}}   
%     %\todo{external reputation score replaces `Q-score';  `internal employee stress score' replaces `stress score'. `stock valuation' replaces `stock value'} } 
%     %\todo{1. possibly define what stock value is. 2. double check all the metrics that they are defined with the right inputs, e.g.,  C and t} \todo{change color scheme} \todo{pFake(T) = number ... in T; $p(T_{all})$ $p(T_{month})$  $p(T_{year})$}} %\todo{add a stock value that is on the monthly resolution.} \todo{add pFake, stress score, stock value, Q-score}} %\todo{add the distribution of shocks of number per company}} % \todo{positive mentions on social media and stress mentions by employees.}
%     \label{tab:res_metrics}
% \end{table*}



% %\subsection{Computing Company Metrics}
% %\todo{report ALL METRICS USED BY ALL RESEARCH QUESTIONS} %\todo{add an misinformation shock metric in Table 2}
% For each company we collated nine metrics, with their formulas and descriptions listed in Table \ref{tab:res_metrics}:
% \begin{itemize}
%   \item \texttt{\# Reddit comments}: we used the total number of Reddit comments discussing a company as a proxy for its popularity among the general public. To make sure that this measure does not capture simply the size of the company, we also tested a corrected metric for popularity:
%   \item \texttt{\# Reddit comments per capita}: calculated as the total number of Reddit comments divided by the total number of Glassdoor reviews (which is a reasonable proxy for the number of employees); 
%   \item \texttt{external reputation score}: as a proxy for public perception of a company, we computed what we call \texttt{Q-score} \cite{freeman1993measuring} (one minus the fraction of the number of comments with a negative sentiment to the total number of comments mentioning the company). To measure the sentiment of a comment, we used the Flair deep learning library \cite{akbik2019flair}, and applied it to \emph{all} the comments mentioning the company, and not only those with a news link;
%   \item \texttt{Glassdoor rating}: as a proxy for the internal perception, i.e., the company's popularity among the (former) employees we calculated the average rating from the company reviews on Glassdoor; 
% \item \texttt{internal employee stress score}: as a proxy for stress mentions by employees is calculated as the per cent of Glassdoor reviews discussing stress at work. To extract work stress mentions from reviews, we used the MedDL entity extraction module~\cite{scepanovic2020extracting}. MedDL uses \emph{contextual embeddings} and a \emph{deep BiLSTM-CRF sequence labeling architecture} (we used the default parameters as specified in~\cite{scepanovic2020extracting}).
% The model was pre-trained and evaluated on a labeled dataset of \newtext{1977} Reddit posts \newtext{(that have in total 4485 medical mentions)} called MedRed~\cite{scepanovic2020extracting}.
% \newtext{The MedRed dataset was split into train (50\%), dev (25\%), and test (25\%) sets. The MedDL method achieved a strict/relaxed $F1$-score of $.71$/$.85$ when extracting symptoms, outperforming two de-facto baselines, MetaMap \cite{aronson2010overview} and TaggerOne \cite{leaman2016taggerone} by a large margin (the two have $F1$-scores of $.17/.48$ and $.31/.58$, respectively).} MedDL has shown generalizability when applied on data from platforms different than those it was trained on, \newtext{including dream reports \cite{vscepanovic2022epidemic} and Glassdoor reviews \cite{vscepanovic2021pressure}};
% % \item  \texttt{stock growth}: as a proxy for external investor perception and valuing of the company is calculated as the ratio of the \texttt{stock valuation} (average adjusted closing prices) in 2019 and 2014.  
% % % prior ai
% % %We considered the growth between these two years because (i) they encompass the Reddit comments posting dates, and having the stock growth starting date in 2014, i.e., two years before the earliest Reddit comments in our data (from 2016), allowed for the company growth rate to be known to the Reddit users at that time, and (ii) focusing on long-term rather than short-term growth increases the metric robustness to the potential influence of external events such as market manipulation, or incidental growth/decline~\cite{forbers21}; 
% % % ai
% %  We chose to focus on the growth of the companies between these two years for two reasons: (i) it encompasses the posting dates of the Reddit comments in our data, thus providing a relevant time frame for examination. Additionally, by selecting a stock growth starting date of 2014, two years prior to the earliest Reddit comments in our dataset from 2016, it allows for the determination of the company's growth rate as it would have been known to Reddit users at that time; (ii) by focusing on long-term growth rather than short-term growth, we increase the robustness of the metric to potential influences of external events such as market manipulation or incidental growth/decline~\cite{forbers21};
%  \item \texttt{pFake}: we computed the probability of news about the company being fake as the ratio of fake to total Reddit comments discussing the company; and finally
%  \item \texttt{misinformation shock}: we calculated as the number of months with \texttt{pFake$(C, T_{month})$ } above its mean and standard deviation within the entire period $T$ for that company.
% \end{itemize}
% We calculated those metrics for the entire time period $T_{all}$ between 2016 and 2019.
% The four metrics that had heavy-tailed distributions (\texttt{\# Reddit comments}, \texttt{\# Reddit comments per capita}, \texttt{stock growth} and \texttt{pFake}) were log-transformed in the further analyses. 
 

% %The MedRed dataset was split into train (50\%), dev (25\%), and test (25\%) sets. 
% %We evalued MedDL using the strict and relaxed $F1$-scores, two commonly used performance metrics for entity extraction models. The \emph{strict $F1$-score} counts only the \emph{exact} matches with the true labels as correct, while the \emph{relaxed $F1$-score} takes into account the partially matching extracted entities. The formulae for the two scores are show in Equation (1). 

% %Finally, we define \texttt{misinformation shock} metric based on the a set of \texttt{pFake} measurements over time series. It is calculated as the number of data points (months) within the entire time series where their \texttt{pFake} is above 2 standard deviations of the mean of \texttt{pFake} within the entire periods $T_{all}$ (between 2016 and 2019).



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{How to categorize corporate fake news articles?}
% % GOAL: Which types of corporate news articles are fake?

% % determine the types of articles
% % determine which are fake: (1) bias of news articles due to company popularity; (2) representativeness of news articles relating to big collusive misinformation event.
% % 

% %So far we have expanded our understanding of the relationships between targeted companies and fake news outlets and when they happen.
% %So far we have established which companies are target of fake news and when (\emph{RQ1-2}). 
% %Other than identifying the creators of fake news (i.e., news outlets), 
% It has been suggested in prior work that identifying the intentions behind the news outlet covering the fake news is crucial to combat it \cite{tandoc2019facts, kalsnes2018fake}.  
% Therefore, we investigate the fake news article categories (\emph{RQ1}): \emph{how do we categorize corporate fake news articles?}

% %\emph{what categories of news articles do fake news outlets cover?}


% To answer this research question, \newtext{we started from an existing taxonomy of fake news article categories in prior literature and expanded it by conducting annotations to identify all the categories (\S\ref{sec:artitletype}). Second, we annotated all the articles during misinformation shocks with the identified categories (\S\ref{sec:study}), and reported the resulting categories in \S\ref{sec:results}.}




% %to establish the of article types
% %we conducted a crowd-sourcing user study by asking users to categorize the fake news articles based on its intention.


% % GOAL: In which articles companies are targeted by fake news?
% % 1. in order to we define an initial article type taxonomy by literature review
% % 2. we select a set of news articles for small-scale lab-based study to define the refined article type taxonomy
% % 3. we run a large-scale crowd-sourcing user study to collect the labels for a set of company related news articles according to the refined artile type taxonomy (in 2).




% % \subsection{Article types}
% \subsection{Identifying  Categories}
% \label{sec:artitletype}

% Several studies \cite{pennycook2021psychology, lazer2018science, kalsnes2018fake, zhou2020survey} investigated the underlying intention, and motivation for creating and spreading fake news. For example, \citet{zhou2020survey} classified the intention of fake news into three categories: mislead, entertain and undefined. \citet{kalsnes2018fake} categorized the motivations of creating fake news into three types: political (spreading their world's view), financial (making money), and social (trolling for fun). Although those taxonomies shed insights on general intentions behind fake news, it is still unclear how that could be translated into a more fine-grained taxonomy of the categories of corporate fake news articles.

% Through a qualitative study, to move beyond those general intention taxonomies, we run an annotation study.
% %
% %and collect the corporate fake news article categories by asking annotators to read the selected fake news stories from those news outlets and then provide the category annotations through coding.
% %
% %\subsubsection{Small-scale Annotations}
% %Firstly, the initial news article categories were motivated by the intention taxonomy from prior literature \cite{pennycook2021psychology, lazer2018science, kalsnes2018fake, zhou2020survey}. 
% %Secondly, 
% Three annotators were instructed to separately annotate the categories for a set of selected news articles independently and to do so with the intention taxonomy from prior literature \cite{pennycook2021psychology, lazer2018science, kalsnes2018fake, zhou2020survey}. %conducting qualitative coding of the subset of the news articles on their intentions. 
% Finally, the annotators discussed their labels to reach the final agreement on a  taxonomy. 
% %until no further categories can be derived for the selected news articles.
% %In the end, we propose the following article categories for corporate fake news, as shown in Table \ref{fig:taxonomy} (level 1 and 2). We found companies that were targeted by fake news tended to be mentioned in articles mainly covering 
% As shown in Table \ref{fig:taxonomy} (level 1 and 2), we found articles were mainly categorized as covering politics, societal issues, products, brands, and corporate affairs. 
% %Note that this news article taxonomy is not intended to be comprehensive due to the nature of our small-scale annotations of the selected news articles. However, this serves as a basis for us to quantify the category distributions for a larger set of fake news articles. We also include a category of ``Others'' for users to specify those categories that were not covered by this initial taxonomy.
% To this taxonomy, we added a category of ``Others'' to specify additional categories.


% \begin{table}[t]
% \caption{\refine{Companies that are targeted by fake news tend to be mentioned in articles mainly covering politics, societal issues, products, brands, and corporate affairs. The top 3 and bottom 3 categories that are widely covered by news outlets are in bold and italic respectively. \newtext{For each category, the top 1 moral dimension with the highest absolute morality score is shown.} \refine{A company that is targeted by fake news tends to be judged with moral dimensions of being unfair (i.e.,~negative fairness), followed by being morally wrong (i.e.,~negative purity) and being harmful (i.e.,~positive harm).}} 
% \includegraphics[width=0.45\textwidth]{figs/taxonomytable3.png}
% \label{fig:taxonomy}
% \end{table}



% %\begin{figure}[t]
% %\centering
% %\includegraphics[width=0.4\textwidth]{figs/taxonomytable2.png}
% %\caption{\refine{Companies that are targeted by fake news tend to be mentioned in articles mainly covering politics, societal issues, products, brands, and corporate affairs. The top 3 and bottom 3 categories that are widely covered by news outlets are in bold and italic respectively. The top 1 judged moral dimension (based on the average dimension score) is shown.} \refine{A company that is targeted by fake news tends to be judged with moral dimensions of being unfair (i.e.,~negative fairness), followed by being impure (i.e.,~negative purity) and being harmful (i.e.,~positive harm).}}

% %\todo{change to latex format}
% %\todo{percentage of articles per category
% %rank the bar plots by level 1 category; then rank by level 2.}
% %\todo{add percentages from figure 7 and make the the top 3 and bottom 3 (sub)categories in bold} } %Intention taxonomy of corporate fake news capturing the types of news articles fake news outlets cover based on their underlying intentions and motivations to target companies.}
% %\label{fig:taxonomy}
% %\end{figure}





% % GOAL: In which articles companies are targeted by fake news?
% % 1. in order to we define an initial article type taxonomy by literature review
% % 2. we select a set of news articles for small-scale lab-based study to define the refined article type taxonomy
% % 3. we run a large-scale crowd-sourcing user study to collect the labels for a set of company related news articles according to the refined artile type taxonomy (in 2).











% % 

% % \subsection{Crowd-sourcing user study}
% \subsection{Annotating Articles with Categories}
% \label{sec:study}

% %To gather more comprehensively the news article categories of corporate fake news on a large-scale, we gathered annotations through a crowdsourcing study via Amazon Mechanical Turk. 

% We then used the taxonomy to label salient news articles with a crowd-sourcing approach.

% \mbox{ } \\ \noindent  
% \textbf{Identifying articles during  misinformation shocks.} Firstly, we selected representative fake news articles that covered the companies of interest. 
% %The intuition behind is to find those news articles that spread across major concentrated fake news attack coverage for a set of companies.
% %
% %
% %\todo{why shock matters}
% %
% %
% %
% %\begin{itemize}
% %\item {\bf \emph{Misinformation Peak Detection.}} 
% We defined representative fake news articles as those shared during ``misinformation shocks'' (as defined in \S3). 
% %
% %An example of identified `misinformation shocks' of the company `Google' is shown in Figure \ref{fig:shock}.
% %\item {\bf \emph{News Article Extraction.}} 
% %
% To overcome the issue of the most popular companies dominating our results,  
% %and therefore biasing selected news articles, 
% we adopted the following strategy: (a)~we randomly selected a company $C$; (b)~we extracted a random set of $k$ articles about company $C$ shared during those months of misinformation shocks; 
% %\todo{point b is not clear, rewrite} 
% (c)~we iterated the previous two steps until all news articles for annotations were collected.
% %\end{itemize}

% After selecting those representative fake news articles, we obtained a random sample of trustworthy news articles (i.e.,~those were not from fake news domains) from the same peak periods. This enabled us to compare two types of news articles, i.e.,~fake and trustworthy.

% \mbox{ } \\ 
% \noindent \textbf{Crowd-sourcing data collection.}
% \newtext{We conducted our crowd-sourcing annotations of news articles according to the taxonomy through Amazon Mechanical Turk.}
% %We ensured that all the participants were paid at least the minimum wage throughout the study.} 
% The data collection consisted of three main steps.
% %questions, and resulted in the generation of two datasets containing annotations for: (a)~\emph{misinformation} news stories, and (b)~\emph{trustworthy} news stories.
% %The three steps of our data collection unfolded as follows.
% %
% First, participants completed a short \emph{pre-study questionnaire} in which they self-reported their age and gender.
% %\footnote{To preserve anonymity, age and gender are the only demographic information we collected.}. 
% %
% Second, the participants were instructed to read the news article in detail.
% %
% %
% Third, participants were instructed to \emph{respond} to answer three questions:
% %the news stories and answer an \emph{questionnaire} to categorize the news stories according to which categories the given company was targeted by the news outlet. 
% %The questionnaire consists of the following questions:
% %\todo{change the itemize as Q to enumerate}
% \begin{description}
% \item \emph{Q1:} Which company does this article mainly cover?
% \item \emph{Q2:} Under which section of corporate coverage would you classify this article?
% \item \emph{Q3:} How would you judge the company based on the article (assuming it is true)? \newtext{Please pick five words each from a different moral dimension.}
% \end{description}
% \emph{Q1} served to collect the company names at hand, and also served as a trap question for us to assess the annotation quality. For those annotators who failed more than one trap question, all their annotations were removed from the analysis. \emph{Q2} collected the categories of our representative articles (as shown in Table \ref{fig:taxonomy}). \newtext{If the assessors could not find any category applicable, they could add their own categorization through a free-text form under the option ``Others''. \emph{Q3} assessed a company would be judged in the article were to be true along the five moral  %focused on morality assessments of the users with five 
% dimensions \cite{graham2011mapping}: harm, fairness, loyalty, authority and purity. The intuition is to identify %users' perceived moral judgments of those companies after reading those fake news articles. The words used to describe each moral dimension can be found in Figure \ref{fig:moral}. 
% these words that were associated to five moral dimensions, with each dimension included two positive and two negative words (Figure \ref{fig:moral}). 
% We then compute the morality score of each moral dimension by counting the corresponding number of positive words selected minus the number of negative words selected.}
% %We computed the average rating with all the moral dimensions.
% %(i.e., the average answer to each of the moral dimensions). 
% %\todo{this last sentence unclear -- can be shortened?}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=0.45\textwidth]{figs/moral.png}
% \caption{Moral dimensions~\cite{graham2011mapping} along which our participants judged a company mentioned in news articles.}
% \label{fig:moral}
% \end{figure}


% \subsection{Popular Categories During Misinformation Shocks}
% \label{sec:results}



% %\todo{read sec 6.3 and see if orders make sense.}
% \noindent \textbf{Categories of Fake News Articles.}  
% %\todo{coverage is not a good word. it should be \% articles in category}
% %We show in Table \ref{fig:taxonomy} (\% Articles in Category) the distribution of the number of fake news articles in the categories.
% %the article categories of our selected fake news articles.
% %, showing the percentage of what news articles cover. 
% %The top 3 and bottom 3 categories (Table \ref{fig:taxonomy} (\% Articles in Category) in bold and italic respectively. For example, ``Product-Issues-Quality'' shares an overall $9.9\%$ of fake news coverage. 
% %We can observe that 
% The top three categories for corporate misinformation are: Product–Issues–Quality, followed by Politics–Lobbying and Product–Launches (Table \ref{fig:taxonomy}). When examining the top high-level (Level 1) categories, ``product'' related fake news is the most frequent, followed by political and societal issues. %are also common categories.
% Interestingly, the option of ``Others'' only was  %is not popular and only covers the 
% 9.7\% 
% %of categories 
% of fake news articles. This partially validated our taxonomy, demonstrating that over 90\% fake news articles are covered by it.

% %\todo{logical jump, thinking about connections.} 
% %In terms of moral dimension, 
% %To assess users' perceived moral judgments on those different categories of fake news articles, 
% %By assessing users' perceived moral judgments of the company after reading the fake news article (Morality in Table \ref{fig:taxonomy}), 
% \newtext{We observe that a company that is targeted by fake news tends to be judged as being unfair (negative fairness), morally wrong (negative purity) and harmful (positive harm).}
% %with the morality of being unfair (negative fairness), followed by being impure (negative purity) and being harmful (positive harm). 
% \newtext{Not surprisingly, for news articles that cover the high-level ``Societal issues'', people perceive them as most morally unacceptable, especially treating them as unfair and doing harm to the society. Comparatively speaking, the ``Societal issues-Minorities-Racial issues'' reflects the most morally wrong categories of news articles that people are disgusted with.
% This demonstrates the impact of fake news to people's moral perception of the company, which could be misaligned with the reality.}
% %\todo{What's the consequence}


% %those categories cover most of the categories (over 90\%) of the corporate fake news articles.
% %The most common descriptions of the ``Others'' are related to Societal issues-Gender (3.4\%), Entertainment-Story/Gossip/Jokes (2.2\%) and Product design (1.8\%).



% %more than 90\% of the news outlet cover news articles belonging to categories that were provided by the options from the category taxonomy derived from the small-scale lab study (\S6.1). This has partially helped validated our news article taxonomy, demonstrating those categories cover most of the categories underlying corporate fake news.




% \begin{comment}
% \begin{figure}[t]
% \centering
% \includegraphics[width=0.4\textwidth]{figs/misinformation_intentionDist.png}
% \caption{\todo{delete} Intention distribution of corporate fake news.}
% \label{fig:dist}
% \end{figure}
% \end{comment}

% \mbox{ } \\
% %\subsubsection{
% \noindent \textbf{How Categories of Fake News Articles Differ from  Trustworthy Ones.} 
% %We calculated the KL divergence of the two category distributions between fake and trustworthy news. We found statistically significant differences of those two distributions ($p<0.01$). This demonstrates that the article categories across the two news article types (fake vs. trustworthy) vary significantly. This validates our hypothesis that when targeting companies, fake news outlets report differently from the trustworthy news outlets.
% %
% %\todo{change c to i}
% To measure the extent to which each category $i$ is associated with fake news as opposed to trustworthy news,  we calculated the \emph{misinformation association $MA(i)$}for each article category $i$:
%     $$MA(i) = \frac{P(i|fake)}{P(i|trustworthy)}$$
% %The higher it is, the more 
% %\todo{odds ratio effect terminology}
% %We found that the higher $MA(c)$, the bigger difference exists in the percentage of targeted coverage article category $c$ between fake and trustworthy news outlets.
% %
% We found that the top 3 categories associated with trustworthy news outlets are ``Brand promotion'', ``Corporate affairs-acquisition'' and ``Politics-regulation'', while the top 3 associated with fake news outlets are  ``Product-Issues-Quality'', ``Politics-Lobbying'' and ``Societal Issues-Conspiracy'' (Table \ref{tab:trust}). 




% %although ``Product–Launches'', ``Brand promotion'' and ``Corporate affairs-strategy'' are the three most popular article categories for trustworthy news outlets, 



% 	\begin{table}[t!]
%         \centering
% 		\caption{Top 3 news article categories with the biggest misinformation effects (the higher the effect is, the larger the difference exists in article categories between fake and trustworthy news outlets).}
% 		\label{tab:effect}
% 		\scalebox{0.75}{\begin{tabular}{lc|lc}
% 			\toprule
% 			\textbf{Top Article Category}&\textbf{News Type }&\textbf{Top Article Category}&\textbf{News Type}\\
% 			\midrule	
% %			Politics - Lobbying &Fake&2.95&Product – Launches&Trustworthy&2.24\\
% %		    books&Fake&1.59&Brand promotion&Trustworthy&1.82\\
% %		    business&Fake&1.50&Corporate affairs - strategy&Trustworthy&1.39\\
% 			 Product-Issues-Quality &Fake&Brand promotion&Trustworthy\\
% 		    Politics-Lobbying&Fake&Corporate affairs-Acquisition&Trustworthy\\
% 		    Societal Issues-Consipiracy&Fake&Politics-regulation&Trustworthy\\

% 		    \bottomrule
% 		\end{tabular}}
%   \label{tab:trust}
% 	\end{table}





% %The popular companies commented a lot on Reddit are those which are more susceptible to fake news relating to ``Product Issues'' and ``Societal Issues'', whereas less popular companies are more likely to deal with ``Politics Lobbying''. 

% %Those companies with higher stock growth are more likely to be targeted by fake news outlets on all the three most popular intentions. This indicates that fake news outlets tend to cover most popular and controversial topics for high-growth companies.

% %However, those companies that were perceived worse internally by employees (i.e., with lower Glassdoor rating) are more susceptible to misinformation on ``Politics Lobbying''. A close examination reveals that ``Politics Lobbying'' are more likely to be targeted specifically to a set of less popular companies (e.g., pharmaceutical companies).





% % \mbox{ } \\ \noindent
% % \textbf{Probability of Being Targeted by Specific News Article Category.} 

% %\todo{reporting median and standard deviation high variability across the months because of these peaks}

==> 7conclusion_saved.tex <==

\section{\newxtext{Discussion}}

%\subsection{Limitations}
Our study has four limitations. First, our attribution of fake news is not at the level of %the news 
article but at that of %the news 
outlet. 
%The fake news used in this paper were based on credibility of the news outlet domain, collected through fact-checking organizations. Although this fake news identification strategy has been widely used in prior research \cite{jahng2021fake, kogan2019fake} in part because it is almost impossible to cover all fake news at the level of individual articles, inevitably it can suffer from: (a) some low-credibility news outlets cover a mix of factual and false articles and thus not all articles are, for sure, ``fake''; (b) there could be fake news not published on these news outlets. However, a 
A recent study showed that, in aggregate, publisher-level credibility scores are very close to article-level ones~\cite{xu2021corporate}. Specifically, the study compared domain-level to article-level misinformation labeling for corporate fake news, and found similar results.
%Second, the fact-checking organizations can have selection bias in deciding which claims to fact-check. For example, some fact-checking organizations favor stories that they consider newsworthy or significant, potentially leading to a bias toward larger companies. 
\refine{Second, our analysis of company perceptions is based on Reddit and Glassdoor. It is unclear whether the conclusions still hold on other social media and company review platforms. Specifically, Reddit is an anonymous platform without the concept of `friends', unlike many other social networks. As such, this platform is missing social pressure, and users are less likely to enter echo chambers, which means that misinformation spreading is not as likely to stem  from homophily \cite{mcpherson2001birds} at the circle-of-friends level as it is on other social networks.} 
Third, we manually selected a set of representative examples of companies showing the association between misinformation patterns and company characteristics (Figure \ref{fig:shock}), and their covered fake news articles. Although this is informative, it does not establish the causal relationships and can not cover the full spectrum of all companies/industries, which we will leave as future work.
\refine{Fourth, our data did not contain comments that were deleted prior to being collected by~\url{pushshift.io}. As such, we could not examine whether those deleted comments contained news URLs. In particular, comments that were removed by Automoderator (bots) were unavailable to us, as these comments were removed as soon as they were posted. Nevertheless, the Reddit dataset from ~\url{pushshift.io} remains one of the most comprehensive datasets available~\cite{baumgartner2020pushshift}.} 


%\subsection{Implications}
%\cliniccomm{Expand.} 
%Our study has several implications: the insights should be of interest to regulators, business leaders, and investors. 
%We showed in this work that there is a link between misinformation and people's company perceptions both internal and external. 
Although major social media platforms have introduced various features to help social media users discern fake content, still, more work is needed. % to combat corporate fake news. 
%Regulators should adopt effective tools to prevent and detect it, and business leaders need to closely monitor increasingly varied threats on social media and stop fake news at its origin. 
To handle a possible misinformation crisis, company should organize a systematic monitoring system. %on what is being said about the brand, to keep external brand damage minimal. Internal communication with employees is another very important aspect to keep in mind while managing such crisis. 
It is also necessary to start direct and transparent communication with employees as soon the crisis arises as this has been shown to help the company to manage the crisis better and faster \cite{holtom2020tips}. 
%Tools should also be developed to increase investors' awareness of fake news when trading on information from social media. 

\noindent \textbf{Broader perspective, ethics and competing interests.} 
\newtext{We are mindful of how personal identities, expectations, norms, and values may influence our study.
Our datasets (such as Reddit, Glassdoor, stock performance, and news outlet credability) were collected from data sources that are publicly available. For those data that contain personal information (such as Reddit user ID), we anonymized the ID and only processed aggregated data for the analysis. Since researchers had no interactions with human subjects of those data, our ethics review board did not consider this part of our research as human subjects research. 
The only part that involve human subjects was our crowd-sourcing user study while only demographics of the participants were collected. The news articles we provided to the users to categorize were from public online news outlets. We ensured that all the participants were paid at least the minimum wage throughout the study. All our analysis of the user study were also based on aggregated data.}
%\todo{In order to provide a balanced perspective, authors are required to include a statement about the potential broader impact of their work and ethical considerations. Papers without such a statement will be desk-rejected. This statement needs to be presented in a clearly marked paragraph/subsection/section in your paper.
%Authors should take care to discuss both positive and negative outcomes. Authors are also expected to describe steps taken to prevent or mitigate potential negative outcomes. For full papers that have collected new datasets and for dataset papers, discuss ethical considerations in the data collection process, considerations around release of the data, and both potentially positive and negative outcomes of its use by others. Given a community as diverse as ICWSM, the issues related to ethics are likely to vary significantly across submissions. As such, we rely on the authors to determine and cover the aspects most relevant to their work. Several checklists used in the past [ 1 , 2 , 3 ] can provide further guidance to scholars looking for starting points.}

%https://neurips.cc/public/EthicsGuidelines
%https://medium.com/@GovAI/a-guide-to-writing-the-neurips-impact-statement-4293b723f832
%https://www.nature.com/articles/s41562-019-0772-6


%For instance, does the dataset use features or label information about individual names? Did people provide their consent on the collection of such data? Could the use of the data be degrading or embarrassing for some people?

%For instance, if the data was collected from a public forum, were its users asked consent to use the data they produced, and if not, why?

%Mturk ethical considerations: fairness in payment, anonymization, aggregated data usage.


%Figure 4: impact to companies and news outlets??








\section{Conclusion}
\newtext{We focused on understanding misinformation in the context of S\&P 500 companies. Through a combination of large-scale social media and crowd-sourcing quantitative analyses, we found that the fake news outlets tend to cover extensively on products, politics and societal issues when reporting misinformation about a company.
We established the relationship between a company's external and internal perceptions and its likelihood of being targeted by fake news. 
We found that companies that suffer severely from fake news are seen negatively both internally and externally. A company is not targeted by fake news all the time, there are particular times in which a critical mass of fake news about the company emerges.}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Discussion}
% \cliniccomm {[Ali] move some part from conlcusion here}

% \section{Conclusion}
% We focus on understanding misinformation in the context of corporate environment. Through large-scale social media quantitative analysis and crowd-sourcing studies, we established the relationship between a company's external and internal perceptions and its likelihood of being targeted by fake news. 
% We found that companies that suffer severely from fake news are seen negatively both internally and externally. A company is not targeted by fake news all the time, there are particular times in which a critical mass of fake news about the company emerges. In addition, the fake news outlets tend to cover more extensively on products, politics and societal issues when reporting misinformation about a company.


% Our study has several limitations. First, our attribution of fake news is not at the level of the news article but at that of the news outlet. The fake news used in this paper were based on credibility of the news outlet domain, collected through fact-checking organizations. Although this fake news identification strategy has been widely used in prior research \cite{jahng2021fake, kogan2019fake} in part because it is almost impossible to cover all fake news at the level of individual articles, inevitably it can suffer from: (a) some low-credibility news outlets cover a mix of factual and false articles and thus not all articles are, for sure, ``fake''; (b) there could be fake news not published on these news outlets. However, a recent study showed that, in aggregate, publisher-level credibility scores are very close to article-level ones~\cite{xu2021corporate}. Specifically, the study compared using domain-level with article-level misinformation labeling for corporate fake news and found similar results.
% Second, the fact-checking organizations can have selection bias in deciding which claims to fact-check. For example, some fact-checking organizations favor stories that they consider newsworthy or significant, potentially leading to a bias toward larger companies. 
% \refine{Third, our analysis of company perceptions is based on Reddit and Glassdoor. It is unclear whether the conclusions still hold on other social media and company review platforms. Specifically, Reddit is an anonymous platform without the concept of `friends', unlike many other social networks. As such, this platform is missing social pressure, and users are less likely to enter echo chambers, which means that misinformation spreading is not as likely to stem  from homophily \cite{mcpherson2001birds} at the circle-of-friends level as it is on other social networks.} %Hence, misinformation spreading is more likely to stem, not from homophily at the circle-of-friends level (as in other social networks), but from people having like-minded individuals in their locations (e.g., states). } 
% %\todo{shall we cite Lia's work here?}
% Fourth, we manually selected a set of representative examples of companies showing the association between misinformation patterns and company characteristics (Figure 4), and their covered fake news articles. Although this is informative, it does not establish the causal relationships and can not cover the full spectrum of all companies/industries, which we will leave as future work.
% \refine{Fifth, our data did not contain comments that were deleted prior to being collected by~\url{pushshift.io}. As such, we could not examine whether those deleted comments contained news URLs. In particular, comments that were removed by Automoderator (bots) were unavailable to us, as these comments were removed as soon as they were posted. Nevertheless, the Reddit dataset from ~\url{pushshift.io} remains one of the most comprehensive datasets available~\cite{baumgartner2020pushshift}.} %Furthermore, reputable news is unlikely to be removed by moderators, and our observations for true news still showed the prominent role of regional personality and culture, speaking to the robustness of our findings. 
% %\todo{Fifth, we selected a set of representative examples of companies showing }


% %\refine{Fourth, we determined what constitutes misinformation based on publishers and not on individual news articles. This approach is widely used in misinformation studies~\cite{bozarth2020higher}, in part because it is almost impossible to cover all fake news at the level of individual articles. A recent study showed that, in aggregate, publisher-level credibility scores are very close to article-level ones~\cite{xu2021corporate}. Specifically, the study compared using domain-level with article-level misinformation labeling for corporate fake news and found similar results.}
% %\todo{copy and paste Lia's relevant paper reviews: domain based fake news assessments.}

% Our study has several implications: the insights should be of interest to regulators, business leaders, and investors. 
% We showed in this work that there is a link between misinformation and people's company perceptions both internal and external. Although major social media platforms have introduced various features to help social media users discern fake content, still, more action is needed to combat corporate fake news. Regulators should adopt effective tools to prevent and detect it, and business leaders need to closely monitor increasingly varied threats on social media and stop fake news at its origin. To be ready to handle a possible misinformation crisis, the company should organize a systematic monitoring system on what is being said about the brand, to keep external brand damage minimal. Internal communication with employees is another very important aspect to keep in mind while managing such crisis. It is necessary to start direct and transparent communication with employees as soon the crisis arises as this has been shown to help the company to manage the crisis better and faster \cite{holtom2020tips}. 
% Tools should also be developed to increase investors' awareness of fake news when trading on information from social media. 



==> figs/5experiment2.tex <==

\section{When companies are targeted by fake news?}


%\todo{to be done}
So far we have expanded our understanding of the relationships between targeted companies and fake news outlets (RQ1). We are now interested in answering \emph{when} companies are targeted by fake news. It was found in previous studies that misinformation can be conducted in a collusive manner \cite{ng2021does, muzykant2021fake}. It is of our particular interest to find when companies suffer from ``misinformation shocks'', which are defined as concentrated periods (e.g., weeks or months) that are targeted by many fake news articles. 

We define representative fake news articles as those articles that cover a given company's major `misinformation shocks'. Specifically, we identify misinformation peaks for a companies in its monthly time series data by finding those months that have their \emph{pFake} being above 2 standard deviations of the mean of \emph{pFake} within the entire periods. 
An example of identified `misinformation shocks' of the company `Google' is shown in Figure \ref{fig:shock}.




%\section{What's the intent behind corporate fake news?}
\section{In which articles companies are targeted by fake news?}

So far we have expanded our understanding of the relationships between targeted companies and fake news outlets. Other than identifying the creators of fake news (i.e., news outlets), it has been suggested that identifying the intentions behind the fake news is crucial to combat it \cite{tandoc2019facts, kalsnes2018fake}.  
Therefore, we further investigate the underlying intentions of fake news articles, i.e., \emph{what types of news articles do fake news outlets cover?}


To answer this research question, we conducted a crowd-sourcing user study by asking users to categorize the fake news articles based on its intention.

\subsection{News article selection}
Firstly, we selected representative fake news articles that covered those companies of interest. The intuition behind is to find those news articles that spread across major concentrated fake news attacks/coverages for a set of companies. 
%\todo{why shock matters}

\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figs/google_misinformation_shock.png}
\caption{\todo{select companies based on storyline and do graph for the full page} \refine{Fake news shocks (peaks of $p_{fake}$ over time) for a company that: has not done well in the stock market (General Electric); attracts more negative mentions on social media (Hartford); attracts more stress mentions by its employees (Newscorp); is a tech company (Facebook and Apple); and is a Communication company (Google).} \refine{Companies are targeted by fake news in specific periods of their existence.}}
\label{fig:shock} 
\end{figure}

\begin{itemize}
\item {\bf \emph{Misinformation Peak Detection.}} We define representative fake news articles as those articles that cover a given company's major `misinformation shocks'. 
Specifically, we identify misinformation peaks for a companies in its monthly time series data by finding those months that have their \emph{pFake} being above 2 standard deviations of the mean of \emph{pFake} within the entire periods. 
%An example of identified `misinformation shocks' of the company `Google' is shown in Figure \ref{fig:shock}.
\item {\bf \emph{News Article Extraction.}} To overcome the issue of the most popular companies dominating and therefore biasing selected news articles, we adopt the following strategy: firstly, we randomly select a company $C$ from all the company pool; secondly, we extract a random pre-defined set of $k$ sub-sample of news articles from the pool of those identified peak months of company $C$; finally we iterate the above two steps until we collect sufficient number of news articles for our annotations.
\end{itemize}

After selecting those representative fake news articles, we obtain a random sample of the trustworthy news articles from the same peak periods. This enables us to compare across those two types of news articles.


\subsection{Article types}

Several studies \cite{pennycook2021psychology, lazer2018science, kalsnes2018fake, zhou2020survey} investigated the underlying intention, and motivation of creating and spreading fake news. For example, \citet{zhou2020survey} classified the intention of fake news into three categories: mislead, entertain and those that are undefined. \citet{kalsnes2018fake} categorized the motivations of creating fake news into three types: political (spreading their world's view), financial (making money) and social (trolling for fun). Although those taxonomies shed insights on general intentions behind fake news, it is still unclear how that could be translated into a more fine-grained intention taxonomy for corporate fake news.

Therefore, through a small-scale qualitative study, we move beyond those general intention taxonomies, and collect the corporate intention taxonomy by asking annotators to read the selected fake news stories from those news outlets and then provide the underlying intention annotations through coding.

%\subsubsection{Small-scale Annotations}
Firstly, the initial intention categories were motivated by prior literature \cite{pennycook2021psychology, lazer2018science, kalsnes2018fake, zhou2020survey}. Secondly, three annotators were instructed to separately annotate the underlying intentions categories for a set of selected news articles (\S5.1), independently conducting qualitative coding of the subset of the news articles on their intentions. 
Finally, annotators discussed their annotations in order to reach the final agreement on the ultimate taxonomy until no further categories can be derived for the selected news articles.
In the end, we propose the following intention taxonomy for corporate fake news, as shown in Figure \ref{fig:taxonomy}.


\begin{figure}[h]
\centering
\includegraphics[width=0.35\textwidth]{figs/taxonomytable2.png}
\caption{\refine{Companies that are targeted by fake news tend to be mentioned in articles mainly covering politics, societal issues, products, brands, and corporate affairs. The top 3 and bottom 3 categories that are widely covered by news outlets are in bold and italic respectively. The top 1 judged moral dimension (based on the average dimension score) is shown.} \refine{A company that is targeted by fake news tends to be judged with positive dimensions of fairness (negative), followed by purity (negative) and harm (positive).}}
%\todo{add percentages from figure 7 and make the the top 3 and bottom 3 (sub)categories in bold} } %Intention taxonomy of corporate fake news capturing the types of news articles fake news outlets cover based on their underlying intentions and motivations to target companies.}
\label{fig:taxonomy}
\end{figure}


Note that this news article coverage type taxonomy is not intended to be comprehensive due to the nature of our small-scale annotations of selected news articles. However, this serves as a basis for us to quantify the distributions for a larger set of fake news articles. We also include a category of ``Others'' for users to specify those categories that were not covered by this initial article type taxonomy.

\subsection{Crowd-sourcing user study}

To gather more comprehensively the intentions of corporate fake news in large-scale, we gathered annotations through a crowdsourcing study via Amazon Mechanical Turk. The data collection consisted of three main questions, and resulted in the generation of two datasets containing annotations for: (a)~\emph{misinformation} news stories, and (b) a ~\emph{trustworthy} news story.
We ensured that all the participants were paid at least the minimum wage throughout the study. The three steps of our data collection unfolded as follows.

First, participants completed a short \emph{pre-study questionnaire} in which they self-reported their age and gender\footnote{To preserve anonymity, age and gender are the only demographic information we collected.}. 

Second, the participants were instructed to read the news article web page in detail.


Third, participants were instructed to \emph{respond} to the news stories and answer an \emph{intention questionnaire} to categorize the news stories according to how the given company was targeted by the news outlet. The questionnaire consists of the following questions:
\begin{itemize}
\item \emph{Q1:} Which company does this article mainly cover?
\item \emph{Q2:} Under which section of corporate coverage you would classify this article?
\item \emph{Q3:} How would you judge the company based on the article (assuming it is true)?
\end{itemize}
\emph{Q1} collects the company the news article mentions, which also serves as a trap question for us to assess the annotation quality. For those careless annotators who failed more than one trap question, all their annotations were removed from the analysis. \emph{Q2} collects  the multi-choice option questions on the intention taxonomy (as shown in Figure \ref{fig:taxonomy}). If the assessors could not find any of the category is applicable, they could add their own categorization through a free-text form under the option ``Others''. \emph{Q3} focuses on morality assessments of the users with five dimensions \cite{graham2011mapping}: harm, fairness, loyalty, authority and purity. The words used to describe each moral dimension can be found in Figure \ref{fig:moral}. These words were associated to five moral dimensions, and each dimension included two positive and two negative words. We computed the average rating with all the moral dimensions (i.e., the average answer to each of the moral dimensions).

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{figs/moral.png}
\caption{Moral dimensions~\cite{graham2011mapping} along which our participants judged a company mentioned in news articles.}
\label{fig:moral}
\end{figure}


\subsection{Experimental Results}

\subsubsection{Fake news outlet coverage}


We show in Figure \ref{fig:taxonomy} the distribution of the coverage categories behind our selected fake news articles, showing the percentage of news outlet coverage. The top 3 and bottom 3 categories are in bold and italic respectively. For example, ``Product-Issues-Quality'' shares an overall $9.9\%$ of fake news coverage. We can observe that:
\begin{itemize}
\item More than 90\% of the news outlet coverage categories are based on provided options in the taxonomy (\S6.2). This has partially helped validated our news coverage taxonomy, demonstrating our taxonomy of news outlet coverage resulted from a small-scale dataset covers most of the categories underlying corporate fake news.

\item The top three underlying categories for corporate misinformation are: Product–Issues–Quality, followed by Politics–Lobbying and Product–Launches. When examining the top high-level categories, ``product'' related fake news is the most frequent type of misinformation news coverage, whereas political and societal issues are also common underlying intentions.

\item For the 9.7\% of coverage categories that were not covered by our taxonomy, the most common coverage categories provided by assessors are: Societal issues-Gender (3.4\%), Entertainment-Story/Gossip/Jokes (2.2\%) and Product design (1.8\%).

\item In terms of moral dimension, a company that is targeted by fake news tends to be judged with positive dimensions of fairness (negative), followed by purity (negative) and harm (positive). Not surprisingly, for news articles that cover the high-level ``Society issues'', the morality scores are quite low, especially for the moral dimensions of fairness and harm. Comparatively speaking, the ``Society issues-Minorities-Racial issues'' reflects the lowest moral judgments overall.
\end{itemize}


\begin{comment}
\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figs/misinformation_intentionDist.png}
\caption{\todo{delete} Intention distribution of corporate fake news.}
\label{fig:dist}
\end{figure}
\end{comment}


\subsubsection{Comparisons of news outlet coverage categories between fake and trustworthy news}

In order to compare the underlying intentions between fake and trustworthy news, we compare the two intention distributions collected from the same set of sampled companies and peak periods.

First of all, we calculate the KL divergence of the two intention distributions between fake and trustworthy news. We found statistically significant differences of those two distributions ($p<0.01$). This demonstrates that the underlying intentions across the two news articles categories vary significantly. This validates our hypothesis that when targeting companies, fake news outlets report significantly different from the trustworthy news outlets.

Secondly, to measure the impacts of targeting intention strategies with different levels of misinformation (fake vs. trustworthy), we calculate the \emph{misinformation effect (ME)}, $ME(i)$, for each article coverage category $i$ as:
    $$ME(i) = \frac{P(i|fake)}{P(i|trustworthy)}$$
where $ME(i)$ measures the \emph{misinformation effect} of the article coverage category $i$. The results of top 3 coverage categories for fake and trustworthy are shown in Table \ref{tab:effect}.
The higher the effect $ME(i)$ is, the bigger difference exists in the percentage of targeted coverage article type $i$ between fake and trustworthy news outlets.

We can observe that: 
\begin{itemize}
\item Although ``Product–Launches'', ``Brand promotion'' and ``Corporate affairs-strategy'' are the three most popular article types for trustworthy news outlets, the actual top 3 article types of trustworthy news outlets that differ from the fake news outlets are: ``Brand promotion'', ``Corporate affairs-acquisition'' and ``Politics-regulation''.
\item On the other hand, fake news outlets generally target more regarding ``Product-Issues-Quality'', ``Politics-Lobbying'' and ``Societal Issues-Conspiracy''.
\end{itemize}

%\todo{intention change to news outlet coverage category}

	\begin{table}[b]
        \centering
		\caption{Top 3 news article coverage type categories with the biggest misinformation effects (the higher the misinformation effect is, the bigger difference exists in the percentage of targeted article type between fake and trustworthy news outlets).}
		\label{tab:effect}
		\scalebox{0.75}{\begin{tabular}{lc|lc}
			\toprule
			\textbf{Top Intention Category}&\textbf{News Type }&\textbf{Top Intention Category}&\textbf{News Type}\\
			\midrule	
%			Politics - Lobbying &Fake&2.95&Product – Launches&Trustworthy&2.24\\
%		    books&Fake&1.59&Brand promotion&Trustworthy&1.82\\
%		    business&Fake&1.50&Corporate affairs - strategy&Trustworthy&1.39\\
			 Product-Issues-Quality &Fake&Brand promotion&Trustworthy\\
		    Politics-Lobbying&Fake&Corporate affairs-Acquisition&Trustworthy\\
		    Societal Issues-Consipiracy&Fake&Politics-regulation&Trustworthy\\

		    \bottomrule
		\end{tabular}}
	\end{table}




\subsection{Probability of being targeted by specific article coverage type}

% p(article type | fake)

%intention vs. Reddit comments per capita, Q-score and stress
\begin{table*}[h]
\centering
\caption{The beta coefficients of the linear regression predicting $p(article\_type | fake)$ for three types of articles.  \refine{Companies targeted by fake news attract more comments on Reddit. However, those that are mentioned in conjunction with product and societal issues do well in the stock market as they are tech companies such as Apple, while those that are mentioned in conjunction with political lobbying tend to do worse among their employees  (in terms of their company review ratings) and typically are pharmaceutical companies such as Pfizer}. Significant values are marked with * based on their significance levels $p<0.05$.} 
     \begin{tabular}{l|c|c|c}
          {\bf Feature}   & \emph{Product Issues} & \emph{Politics Lobbying} &  \emph{Societal Issues} \\  \hline
        Intercept & -1.22*  & -2.14*  & -1.87*  \\ 
        \# Reddit comments per capita & 2.41* & -0.73 & 1.63* \\ 
        Q-score & -0.35 & 0.72 & -0.55  \\ 
        Glassdoor rating & -0.89 & -1.24* & -0.76  \\ 
        stress score & 0.12 & 0.24 & -0.10 \\  
        stock growth & 1.45* & 0.54  & 1.02*  \\\hline
    \end{tabular}
    \label{tab:models}
\end{table*}

We calculated the probability of fake news targeting the top 3 specific news article coverage types: product issues, politics lobbying, and societal issues, and investigated which company characteristics influence this probability mostly. 
To answer this question, we ran a linear regression with intention probability as the dependent variable and our metrics listed in Table 2 as independent variables.
Specifically, we ran three linear regression models, with the
following sets of independent variables (\S4.1): \# Reddit comments per capita, stress score, Q-score, stock growth and Glassdoor rating.
%
%
We can observe that:
\begin{itemize}
\item Those popular companies commented a lot on Reddit are more susceptible to fake news relating to ``Product Issues'' and ``Societal Issues'', whereas less popular companies are more likely to deal with ``Politics Lobbying''. 
\item Those companies perceived worse internally by employees (i.e., with lower Glassdoor rating) are more susceptible to misinformation on ``Politics Lobbying''. A close examination reveals that ``Politics Lobbying'' are more likely to be targeted specifically to a set of less popular companies (e.g., pharmaceutical companies).
\item Those companies with higher stock growth are more likely to be targeted by fake news outlets on all the three most popular intentions. This indicates that fake news outlets tend to cover most popular and controversial topics for high-growth companies.
\end{itemize}
